Fairness Testing: A Comprehensive Survey and Analysis of Trends

Unfair behaviors of Machine Learning (ML) software have garnered increasing attention and concern among software engineers. To tackle this issue, extensive research has been dedicated to conducting fairness testing of ML software, and this paper offers a comprehensive survey of existing studies in this field. We collect 100 papers and organize them based on the testing workflow (i.e., how to test) and testing components (i.e., what to test). Furthermore, we analyze the research focus, trends, and promising directions in the realm of fairness testing. We also identify widely-adopted datasets and open-source tools for fairness testing.

==> macro.tex <==
\definecolor{darkpastelgreen}{rgb}{0.20, 0.40, 0.20}
\definecolor{darkpastelred}{rgb}{0.80, 0.20, 0.20}
\definecolor{amber}{rgb}{0.7, 0.5, 0}
\definecolor{tablegray}{gray}{0.92}


% tech name
\newcommand{\UniStarDeepfl}{\deepfl\textsubscript{\uniaprtwostar{}}}
\newcommand{\unideepfl}{\deepfl\textsubscript{{\uniaprtwo{}}}}
\newcommand{\uniprfl}{\prfl\textsubscript{\uniaprtwo{}}}

% \newcommand{\UniStarPrfl}{\uniapr\textsuperscript{*}\textsubscript{\prfl}}
\newcommand{\UniStarPrfl}{\uniaprtwostar{}\textsubscript{\prfl{}}}
\newcommand{\uniprfla}{\prflma\textsubscript{\uniaprtwo}}
% \newcommand{\UniStarPrfla}{\uniapr\textsuperscript{*}\textsubscript{\prfl MA}}
\newcommand{\UniStarPrfla}{\prflma\textsubscript{\uniaprtwostar{}}}

\newcommand{\praprprfl}{\profl\textsubscript{\prfl}}

% \newcommand{\PraprStarPrfl}{\profl\textsuperscript{*}\textsubscript{\prfl}}
\newcommand{\PraprStarPrfl}{\proflstar{}\textsubscript{\prfl}}

\newcommand{\praprprfla}{\profl\textsubscript{\prfl{} MA}}

% \newcommand{\PraprStarPrfla}{\profl\textsuperscript{*}\textsubscript{\prfl MA}}
\newcommand{\PraprStarPrfla}{\proflstar{}\textsubscript{\prfl{} MA}}

% \newcommand{\PraprStardeepfl}{\profl\textsuperscript{*}\textsubscript{\deepfl}}
\newcommand{\PraprStardeepfl}{\proflstar{}\textsubscript{\deepfl{}}}

\newcommand{\deepfl}{DeepFL}
\newcommand{\prfl}{PRFL}
\newcommand{\prflma}{PRFL\textsubscript{MA}}
\newcommand{\fl}{fault localization}
\newcommand{\muse}{MUSE}
\newcommand{\meta}{Metallaxis}
\newcommand{\sbfl}{spectrum-based fault localization}
\newcommand{\apr}{APR}
\newcommand{\uniapr}{UniDebug}
\newcommand{\unidebugU}{Unified Debugging}
\newcommand{\unidebug}{unified debugging}

% dataset
\newcommand{\dfts}{Defects4J}
\newcommand{\lang}{Lang}
\newcommand{\chart}{Chart}
\newcommand{\ctime}{Time}
\newcommand{\cmath}{Math}
\newcommand{\mockito}{Mockito}
\newcommand{\closure}{Closure}

\newcommand{\jdkshortseven}{JDK 1.7}
\newcommand{\jdklongseven}{JDK 1.7.0.80}

\newcommand{\jdkshorteight}{JDK 1.8}
\newcommand{\jdklongeight}{JDK 1.8.0.242}

\newcommand{\toolNum}{16}
%%%%%%%%%% TOOL MACRO START %%%%%%%%%%
\newcommand{\acs}{ACS}

%% ARJA %%
\newcommand{\arja}{Arja}
\newcommand{\kali}{Kali-A}
\newcommand{\genprog}{GenProg-A}
\newcommand{\rsrepair}{RSRepair-A}
\newcommand{\gprog}{GenProg}

%% ASTOR %%
\newcommand{\cardumen}{Cardumen}
\newcommand{\jgenprog}{jGenProg}
\newcommand{\jkali}{jKali}
\newcommand{\jmutrepair}{jMutRepair}

%% NOPOL %%
\newcommand{\dynamoth}{Dynamoth}
\newcommand{\nopol}{Nopol}

%% TBAR-RELATED %%
\newcommand{\avatar}{AVATAR}
\newcommand{\kpar}{kPar}
\newcommand{\fixminer}{FixMiner}
\newcommand{\tbar}{TBar}
\newcommand{\prophet}{Prophet}
\newcommand{\simfix}{Simfix}
\newcommand{\pit}{PIT}
%%%%%%%%%% TOOL MACRO END %%%%%%%%%%

\newcommand{\profl}{ProFL}
\newcommand{\proflplus}{\sam{CHANGE THIS MACRO!!}\uniaprone{}}
\newcommand{\uniaprone}{\uniapr+}
\newcommand{\uniaprtwo}{\uniapr++}
\newcommand{\uniaprtwostar}{\uniaprone{}$^\star$}
\newcommand{\prapr}{PraPR}
\newcommand{\proflstar}{ProFL$^\star$}

%patches
\newcommand{\cleanfix}{CleanFix}
\newcommand{\cleanfixfull}{\cleanfix$_{Full}$}
\newcommand{\cleanfixpartial}{\cleanfix$_{Partial}$}
\newcommand{\noisyfix}{NoisyFix}
\newcommand{\noisyfixfull}{\noisyfix$_{Full}$}
\newcommand{\noisyfixpartial}{\noisyfix$_{Partial}$}
\newcommand{\nonefix}{NoneFix}
\newcommand{\negfix}{NegFix}
\newcommand{\nonmodify}{Non-Modify}

%\newcommand{\codeIn}[1]{\lstinline!#1!}
\newcommand{\codeIn}[1]{\texttt{#1}}
\newcommand{\parabf}[1]{\noindent \textbf{#1}}

\newcounter{finding}


\newcommand{\finding}[1]{\refstepcounter{finding}
	\begin{figure}[H]
    	\begin{center}
        	\begin{adjustbox}{width=\columnwidth}
        	\vspace{0.5em}
            	\begin{tcolorbox}[colback=gray!15, boxsep=0.0em, arc=0.1em, boxrule=0.05em, colframe=gray]
            		\textbf{Finding \arabic{finding}:} #1
            	\end{tcolorbox}
            	\vspace{0.5em}
        	\end{adjustbox}
    	\end{center}
	\end{figure}
}

\newcommand{\camreview}[1]{{\color{amber}[#1]}}
\newcommand{\camready}[1]{{\color{amber}[#1]}}
\newcommand{\old}[1]{{\color{red}[#1]}}

\newcommand{\sbflformulaecount}{33}
\newcommand{\tablewidth}{0.92\columnwidth}

\lstdefinestyle{javadiff}{
language=JAVA,
basicstyle=\ttfamily\scriptsize,
frame=shadowbox,
morecomment=[f][\color{darkpastelred}][0]{-},
morecomment=[f][\color{darkpastelgreen}][0]{+},
morecomment=[f][\color{gray!75}\textit][0]{/**},
}
